Regularized Submodular Maximization at Scale

In this paper, we propose scalable methods for maximizing a regularized submodular function $f = g - \ell$ expressed as the difference between a monotone submodular function $g$ and a modular function $\ell$. Indeed, submodularity is inherently related to the notions of diversity, coverage, and representativeness. In particular, finding the mode of many popular probabilistic models of diversity, such as determinantal point processes, submodular probabilistic models, and strongly log-concave distributions, involves maximization of (regularized) submodular functions. Since a regularized function $f$ can potentially take on negative values, the classic theory of submodular maximization, which heavily relies on the non-negativity assumption of submodular functions, may not be applicable. To circumvent this challenge, we develop the first one-pass streaming algorithm for maximizing a regularized submodular function subject to a $k$-cardinality constraint. It returns a solution $S$ with the guarantee that $f(S)\geq(\phi^{-2}-\epsilon) \cdot g(OPT)-\ell (OPT)$, where $\phi$ is the golden ratio. Furthermore, we develop the first distributed algorithm that returns a solution $S$ with the guarantee that $\mathbb{E}[f(S)] \geq (1-\epsilon) [(1-e^{-1}) \cdot g(OPT)-\ell(OPT)]$ in $O(1/ \epsilon)$ rounds of MapReduce computation, without keeping multiple copies of the entire dataset in each round (as it is usually done). We should highlight that our result, even for the unregularized case where the modular term $\ell$ is zero, improves the memory and communication complexity of the existing work by a factor of $O(1/ \epsilon)$ while arguably provides a simpler distributed algorithm and a unifying analysis. We also empirically study the performance of our scalable methods on a set of real-life applications, including finding the mode of distributions, data summarization, and product recommendation.

==> tex/proof_distributed.tex <==
\section{Proof of Theorem~\ref{thm:distributed} } \label{appendix-proof-distributed}

Theorem~\ref{thm:distributed} guarantees the performance of  \AlgDistributed (Algorithm~\ref{alg:distributed}).
In this section we first restate and then prove Theorem~\ref{thm:distributed}.

\begin{reptheorem} {thm:distributed}
	\ThmDistributed
\end{reptheorem}

We define the submodular function $f(S) \triangleq g(S) - \ell(S)$. 
It is easy to see that $f$ is a submodular function (although it is not guaranteed to be either monotone or non-negative). The Lov\'asz extension of $f$ is the function $\lov{f}\colon [0,1]^{\cN} \to \bR$ given by
\begin{align*}
\lov{f}(\mathbf{x})=\underset{\theta \in \mathcal{U}(0,1)}{\mathbb{E}}\left[f\left(\left\{i: x_{i} \geq \theta\right\}\right)\right] \enspace,
\end{align*} 
where $\cU(0, 1)$ is the uniform distribution within the range $[0, 1]$~\cite{lovasz1983submodular}. Note that the Lov\'asz extension of a modular set function is the natural linear extension of the function. It was also proved in~\cite{lovasz1983submodular} that the Lov\'{a}sz extension of a submodular function is convex. Finally, we need the following well-known properties of Lov\'asz extensions, which follow easily from its definition.
\begin{observation} \label{obs:basic_properties}
	For every set $S \subseteq \cN$, $\lov{f}(\mathbf{1}_S) = f(S)$. Additionally, $\lov{f}(c \cdot \mathbf{p}) \geq c \cdot \lov{f}(\mathbf{p})$ for every $c \in[0,1]$ and $\mathbf{p} \in [0, 1]^\cN$ whenever $f(\varnothing)$ is non-negative.
\end{observation}

Let us denote by $\AlgDistorted(A)$ the set produced by $\AlgDistorted$ when it is given the elements of a set $A \subseteq \cN$ as input. Using this notation, we can now state the following lemma. We omit the simple proof of this lemma, but note that it is similar to the proof of \cite[Lemma~2]{barbosa2015power}.
\begin{lemma} \label{lemma:lemma:dg-union}
	Let $A \subseteq \cN$ and $B \subseteq \cN$ be two disjoint subsets of $\cN$. Suppose that, for each element
	$u \in B$, we have $\AlgDistorted(A \cup \{u\}) = \AlgDistorted(A)$. Then, $\AlgDistorted(A \cup B) = \AlgDistorted(A)$.
\end{lemma}

We now need some additional notation. Let $S^*$ denote an optimal solution for Problem~\eqref{eq:problem}, and let $\mathcal{\cN}(1 / m)$ represent the distribution over random subsets of $\cN$ where each element is sampled independently with probability $1 / m$. To see why this distribution is important, recall that $\cN_{r, i}$ is the set of elements assigned to machine $i$ in round $i$ by the random partition, and that every element is assigned uniformly at random to one out of $m$ machines, which implies that the distribution of $\cN_{r, i}$ is identical to $\mathcal{\cN}(1 / m)$ for every two integers $1 \leq i \leq m$ and $1 \leq r \leq \eps^{-1}$. We now define for every integer $0 \leq r \leq \eps^{-1}$ the set $C_r = \cup_{r' = 1}^r \cup_{i = 1}^m S_{r', i}$ and the vector $\mathbf{p}^r \in [0,1]^{\cN}$ whose $u$-coordinate, for every $u \in \cN$, is given by
\[ p^r_u=
\begin{cases}
\Pr_{A \sim \cN(1/m)} [u \not \in C_{r - 1} \text{ and } u \in \AlgDistorted(A \cup C_{r - 1} \cup \{u\})] & \text{if } u \in S^* \enspace,  \\
0 & \text{otherwise} \enspace.
\end{cases}
\]
The next lemma proves an important property of the above vectors.
\begin{lemma} \label{lem:sum_p}
	For every element $u \in S^*$ and $0 \leq r \leq 1 / \eps$, $\Pr[u \in C_r] = \sum_{r' = 1}^r p^{r'}_u$.
\end{lemma}
\begin{proof}
	Since $u$ is assigned in round $r'$ to a single machine uniformly at random,
	\begin{align*}
	\mspace{100mu}&\mspace{-100mu}
	\Pr[u \in C_{r'} \setminus C_{r' - 1}]
	=
	\Pr[u \in \cup_{i = 1}^m S_{r', i} \setminus C_{r' - 1}]
	=
	\frac{1}{m} \sum_{i = 1}^m \Pr[u \in S_{r', i} \setminus C_{r' - 1} \mid u \in \cN_{r', i}]\\
	={} &
	\frac{1}{m} \sum_{i = 1}^m \Pr[u \not \in C_{r' - 1} \text{ and } u \in \AlgDistorted(\cN_{r', i} \cup (\cup_{r'' = 1}^{r' - 1} \cup_{i' = 1}^m S_{r'', i'})) \mid u \in \cN_{r', i}]\\
	={} &
	\frac{1}{m} \sum_{i = 1}^m \Pr\nolimits_{A \sim \cN(1/m)}[u \not \in C_{r' - 1} \text{ and } u \in \AlgDistorted(A \cup C_{r' - 1} \cup \{u\})]
	=
	p^{r'}_u
	\enspace,
	\end{align*}
	where the first equality holds since $C_{r'}$ can be obtained from $C_{r'- 1}$ by adding to the last set all the elements of $\cup_{i = 1}^m S_{r', i}$ that do not already belong to $C_{r' - 1}$, and the last equality holds since the distribution of $\cN_{r', i}$ conditioned on $u$ belonging to this set is equal to the distribution of $A \cup \{u\}$ when $A$ is distributed like $\cN(1/m)$.
	
	Since $C_1 \subseteq C_2 \subseteq \dotso \subseteq C_r$, the events $\Pr[u \in C_{r'} \setminus C_{r' - 1}]$ must be disjoint for different values of $r'$, which implies
	\[
	\sum_{r' = 1}^r p^{r'}_u
	=
	\sum_{r' = 1}^r \Pr[u \in C_{r'} \setminus C_{r' - 1}]
	=
	\Pr[u \in C_r] - \Pr[u \in C_0]
	=
	\Pr[u \in C_r]
	\enspace,
	\]
	where the last equality holds since $C_0 = \varnothing$ by definition.
\end{proof}

Using the last lemma, we can now prove lower bounds on the expected values of the sets $S_{r, i}$.
\begin{lemma} \label{lemma:bound-lovasz} 
	Let $\lov{g}$ and $\lov{\ell}$ be the Lov\'asz extensions of the functions $g$ and $\ell$, respectively. Then, for every two integers $1 \leq r \leq \eps^{-1}$ and $1 \leq i \leq m$,
	\begin{align*}
	\bE[f(S_{r, i})] \geq  (1 - e^{-1}) \cdot \lov{g}(\mathbf{1}_{S^*}-\mathbf{p}^r ) - \lov{\ell}(\mathbf{1}_{S^*}-\mathbf{p}^r ) \enspace,
	\end{align*}
	and
	\[
	\bE[f(S_{r, i})] \geq  (1 - e^{-1}) \cdot \lov{g}({\textstyle \sum_{r' = 1}^{r - 1} \mathbf{p}^{r'} }) - \lov{\ell}({\textstyle \sum_{r' = 1}^{r - 1}\mathbf{p}^{r'} })
	\enspace.
	\]
\end{lemma} 
\begin{proof}
	Let $R = \{u \in S^* \mid u \not \in \AlgDistorted(\cN_{r, i} \cup C_{r - 1} \cup \{u\})\}$, and let $O_{r, i}$ be some random subset of $S^*$ to be specified later which includes only elements of $\cN_{r, i} \cup C_{r - 1} \cup R$. By Lemma~\ref{lemma:lemma:dg-union},
	\begin{align*}
	S_{r, i}
	={} &
	\AlgDistorted(\cN_{r, i} \cup (\cup_{r' = 1}^{r - 1} \cup_{i' = 1}^m S_{r', i'}))\\
	={} &
	\AlgDistorted(\cN_{r, i} \cup C_{r - 1})
	=
	\AlgDistorted(\cN_{r, i} \cup C_{r - 1} \cup R)
	\enspace.
	\end{align*}
	Due to this equality and the fact that $|O_{r, i}| \leq |S^*| \leq k$, the guarantee of \AlgDistorted~\cite[Theorem~3]{harshaw2019submodular} implies:
	\[f(S_{r, i}) = g(S_{r, i}) - \ell(S_{r, i}) \geq (1 - e^{-1}) \cdot g(O_{r, i}) - \ell(O_{r, i}) \enspace.\]
	Therefore,
	\begin{align} \label{eq:general_O}
	\bE[f(S_{r, i})] &
	\geq \bE[   (1 - e^{-1}) \cdot g(O_{r, i}) - \ell(O_{r, i}) ] 
	= (1 - e^{-1}) \cdot \bE[  g(O_{r, i}) ] - \bE[ \ell(O_{r, i}) ] \\ \nonumber
	& \geq (1 - e^{-1}) \cdot \lov{g}(\bE[\mathbf{1}_{O_{r, i}}]) - \lov{\ell}(\bE[ \mathbf{1}_{O_{r, i}}]) \enspace,
	\end{align}
	where the second inequality holds since $\lov{g}$ is convex and $\lov{\ell}$ is linear (see the discussion before Observation~\ref{obs:basic_properties}).
	
	To prove the first part of the lemma, we now choose
	\[
	O_{r, i}= (C_{r - 1} \cap S^*) \cup R = (C_{r - 1} \cap S^*) \cup \left\{u \in S^{*}: u \notin \AlgDistorted(\cN_{r, i} \cup C_{r - 1} \cup\{u\})\right\}
	\enspace.
	\]
	One can verify that this choice obeys our assumptions about $O_{r, i}$; and moreover, since the distribution of $\cN_{r, i}$ is the same as that of $\cN(1/m)$, we get:
	\[
	\Pr\left[u \in O_{r, i}\right] =1-\operatorname{Pr}\left[u \notin O_{r, i}\right]=1-p^r_{u} \quad \forall\; u\in S^* \qquad \text{and} \qquad
	\mathbb{E}\left[\mathbf{1}_{O_{r, i}}\right] =\mathbf{1}_{S^*}-\mathbf{p}^r \enspace.
	\]
	The first part of the lemma now follows by combining the last equality with Inequality~\eqref{eq:general_O}.
	
	To prove the second part of this lemma, we choose $O_{r, i} = C_{r - 1} \cap S^*$. One can verify that this choice again obeys our assumptions about $O_{r, i}$; and moreover, by Lemma~\ref{lem:sum_p}, $\bE[\mathbf{1}_{O_{r, i}}] = \sum_{r' = 1}^{r - 1} \mathbf{p}^{r'}$. The second part of the lemma now follows by combining this equality with Inequality~\eqref{eq:general_O}.
\end{proof}
%\begin{lemma} \label{lemma:bound-alg-union}
%For $S = \AlgDistorted(\cup_{i=1}^{m} S_i)$, we have $\bE[f(S)] \geq  (1 - e^{-1}) \cdot g^{-}(\mathbf{p} ) - \ell^{-}(\mathbf{p} )$.
%\end{lemma}
%\begin{proof}
%%	We again point out that the proof of this lemma follows the main ideas of the proof of \cite[Lemma~4]{barbosa2015power}, and they are provided here mainly for the sake of completeness.
%Let us define $S' = \cup_{i=1}^{m}S_i$. 
%From the theoretical guarantee of $\AlgDistorted$ due to \cite{harshaw2019submodular}, we have:
%\begin{align} \label{eq:bound-union}
%f(S) \geq (1 - e^{-1}) \cdot g(S' \cap S^*)  - \ell(S' \cap S^*) \enspace.
%\end{align}
%Additionally, for each machine $i$ and element $u \in S^*$, we have:
%\begin{align*}
%\operatorname{Pr}\left[u \in \AlgDistorted(\cN_{i}) \mid u \in \cN_{i}\right]
%&=\operatorname{Pr}_{A \sim \mathcal{\cN}(1 / (\eps m))}[u \in \AlgDistorted(A) \mid u \in A] \\
%&= \operatorname{Pr}_{B \sim \mathcal{\cN}(1 / (\eps m))}[u \in \AlgDistorted(B \cup\{u\})]
%= p_{u} \enspace,
%\end{align*}
%where the first equality is the result of the fact that the distribution of $\cN_i$
%is the same as $\cN(1/(\eps m))$; and
%the second equality s true because the distribution of $A \sim \cN(1/(\eps m))$ conditioned on the event $u \in A$ is identical to the distribution of $B \cup \{ u\}$, where $B$ is a random set distributed like $\cN(1/(\eps m))$. 
%Therefore, for every set $M$ of $1/\eps$ machines,
%\begin{align*}
%\mspace{100mu}&\mspace{-100mu}
%\Pr[u \in S' \cap S^* \mid \text{$u$ is sent exactly to the machines of $M$}]\\
%={} &
%\Pr[u \in \cup_{i \in M} \AlgDistorted(\cN_{i}) \mid u \in \cN_i \forall\; i \in M]\\
%={} &
%1 - \prod_{i \in M} \left(1 - \Pr[u \in \AlgDistorted(\cN_{i}) \mid u \in \cN_i]\right)
%=
%1 - (1 - p_u)^{|M|}
%\geq
%1 - e^{-p_u|M|}\\
%\geq{} &
%p_u|M| - \frac{p^2_u|M|^2}{2}
%\end{align*}
%\[
%\Pr[u \in S' \cap S^*]
%=
%\sum_{\substack{M \subseteq \{1, 2, \dotsc, m\}\\|M| = 1/\eps}} \Pr[\text{$u$ is sent exactly to the machines of $M$}] \cdot \Pr[u \in \cup_{i \in M} \AlgDistorted(\cN_{i}) \mid u \in \cN_{i} \mid \text{$u$ is sent exactly to the machines of $M$}]
%\]
%\begin{equation} \label{eq:prob-opt}
%\operatorname{Pr}[u \in S' \cap S^*] =p_{u} \qquad \text{and} \qquad
%\bE \left[\mathbf{1}_{S' \cap S^*}\right] =\mathbf{p} \enspace.
%\end{equation}
%Combining \cref{eq:bound-union,eq:prob-opt} and Lemma~\ref{lemma:barbosa-lem1} we get
%\[ \bE[f(S)] \geq (1 - e^{-1}) \cdot \bE[g(S' \cap S^*)] - \bE[\ell(S' \cap S^*)] \geq  (1 - e^{-1}) \cdot g^{-}(\mathbf{p} ) - \ell^{-}(\mathbf{p} ) \enspace. \qedhere \]
%\end{proof}

We are now ready to prove Theorem~\ref{thm:distributed}.
\begin{proof}[Proof of Theorem~\ref{thm:distributed}]
	Let $D$ be the output set of \cref{alg:distributed}. The definition of $D$ and Lemma~\ref{lemma:bound-lovasz}  together guarantee that for every $1 \leq r \leq \eps^{-1} - 1$ we have
	\[
	\bE[f(D)]  \geq \bE[f(S_{r, 1})] \geq  (1 - e^{-1}) \cdot \lov{g}(\mathbf{1}_{S^*}-\mathbf{p}^r ) - \lov{\ell}(\mathbf{1}_{S^*}-\mathbf{p}^r )
	\enspace,
	\]
	and additionally, 
	\[
	\bE[f(D)]  \geq \bE[f(S_{1/\eps, 1})] \geq  (1 - e^{-1}) \cdot \lov{g}({\textstyle \sum_{r = 1}^{1/\eps - 1} \mathbf{p}^r }) - \lov{\ell}({\textstyle \sum_{r = 1}^{1/\eps - 1} \mathbf{p}^r})
	\enspace.
	\]
	Therefore,
	\begin{align*}
	\bE[f(D)]
	\geq{} &
	\eps \cdot \mspace{-3mu} \sum_{r = 1}^{1/\eps - 1} [(1 - e^{-1}) \cdot \lov{g}(\mathbf{1}_{S^*}-\mathbf{p}^r ) - \lov{\ell}(\mathbf{1}_{S^*}-\mathbf{p}^r )] + \eps[(1 - e^{-1}) \cdot \lov{g}({\textstyle \sum_{r = 1}^{1/\eps - 1} \mathbf{p}^r }) - \lov{\ell}({\textstyle \sum_{r = 1}^{1/\eps - 1} \mathbf{p}^r})]\\
	\geq{} &
	(1 - e^{-1}) \cdot \lov{g}\left(\eps \cdot \sum_{r = 1}^{1/\eps - 1}(\mathbf{1}_{S^*}-\mathbf{p}^r) + \eps \cdot \sum_{r = 1}^{1/\eps - 1} \mathbf{p}^r\right) - \lov{\ell}\left(\eps \cdot \sum_{r = 1}^{1/\eps - 1}(\mathbf{1}_{S^*}-\mathbf{p}^r) + \eps \cdot \sum_{r = 1}^{1/\eps - 1} \mathbf{p}^r\right)\\
	={} &
	(1 - e^{-1}) \cdot \lov{g}\left((1 - \eps) \cdot \mathbf{1}_{S^*}\right) - \lov{\ell}\left((1 - \eps) \cdot \mathbf{1}_{S^*}\right)
	\geq
	(1 - \eps) \cdot \left[(1 - e^{-1}) \cdot g(S^*) -\ell(S^*)\right]
	\enspace,
	\end{align*}
	where the second inequality holds since $\lov{\ell}$ is linear and $\lov{g}$ is convex, and the last inequality follows again from the linearity of $\lov{\ell}$ and Observation~\ref{obs:basic_properties} because $f(\varnothing) = g(\varnothing) - \ell(\varnothing) = g(\varnothing) \geq 0$.
\end{proof}
